Matter to Mechanism: A Benchmark for AI Co-Scientists in Materials and Battery Research

AI co-scientists are increasingly used for scientific discovery, but current evaluations still do not test them on a key task: moving from a concrete scientific or technological problem to a plausible, mechanism-grounded solution hypothesis. This gap is especially important in materials science and, in particular, battery research, where a useful proposal must identify the relevant failure mode, propose a credible intervention, and explain why that intervention should improve the target property. We introduce Matter to Mechanism, a benchmark for evaluating AI co-scientists on problem-to-hypothesis reasoning in materials science, with a focus on battery materials research. The benchmark contains 2,645 instances derived from scientific publications. Each instance includes a structured problem statement, a candidate solution hypothesis, an explicit reasoning trace, and domain-grounded annotations such as material system, component, failure mode, intervention, mechanism, target property, and claimed outcome. We also introduce a metric suite that measures reasoning fidelity, problem alignment, mechanistic specificity, novelty, plausibility, and problem decomposition quality, and combine them into a composite score. Using this framework, we evaluate several AI co-scientist systems and show that Matter to Mechanism reveals interpretable system differences that are only partially recovered by standard text-similarity metrics. We further show through adversarial stress tests that the aggregate score is more stable than individual metric dimensions under superficial gaming attacks.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}
 

%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state the paper's main contribution as a benchmark and evaluation framework for problem-to-solution reasoning in materials science, with a focus on battery research. The paper also scopes its claims carefully by stating that \bench{} measures one specific part of scientific reasoning rather than scientific discovery in full, and by presenting the metric suite as a structured evaluation framework rather than a complete measure of scientific quality.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes a dedicated Discussion and Limitations section. It discusses the restricted scope of the benchmark, possible noise from automatic extraction of structured fields, the reliance on hand-designed heuristics and weighted components, the instability of pairwise LLM-judge validation, and the fact that the benchmark does not cover tool selection or experimental planning.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present formal theoretical results such as theorems or proofs. It introduces programmatic evaluation metrics and reports empirical benchmark results.

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper specifies the benchmark size, the compared systems, the evaluation setting, the six metric definitions, the metric weights, the validation setup, and the adversarial attack styles. The appendix gives detailed metric definitions, and the main text explains the benchmark task, system setup, and validation experiments sufficiently to understand and reproduce the reported results.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The current submission provide open access links to the benchmark data and evaluation code in anonymized form. Both the anonymized dataset and code can be found in the submission.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper does not train a new model. For the benchmark experiments, it specifies the systems evaluated, the task input format, the reference-free evaluation setup, the validation subset size, the LLM-judge protocol including swap-order comparison, and the adversarial attack setup. These details are sufficient to understand the empirical setting and interpret the reported results.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The main leaderboard reports 95\% bootstrap confidence intervals for all system-level metric means in Table~\ref{tab:main_results}, computed using 2{,}000 resamples over benchmark instances. The comparison with reference-based metrics also reports Kendall's $\tau$ values with corresponding $p$-values. These statistics provide uncertainty estimates for the main benchmark scores and significance information for the rank-agreement analysis.
    
    \item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Once system outputs are available, the benchmark scoring and validation analyses are lightweight and can be run on a standard CPU node; the full programmatic evaluation pipeline runs in under two minutes. The system-output generation and analysis runs reported in the paper used up to 2 NVIDIA H200 GPUs. Exact runtime may vary across model backends and API availability, but the released scripts reproduce the leaderboard, reference-metric comparison, pairwise judge analysis, metric-gaming test, and ablations.


\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: To the best of our knowledge, the research complies with the NeurIPS Code of Ethics. The benchmark is built from published scientific literature, the paper discusses limitations and possible misuse-related considerations, and no human-subject experimentation is part of the core contribution as currently presented.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: The work is primarily a benchmark for scientific reasoning in materials science research.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not release a high-risk generative model or a scraped internet dataset of the kind typically associated with elevated misuse risk. The contribution is a benchmark and evaluation framework built from published scientific literature.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper cites the existing models, benchmarks, and prior work used for comparison, and documents the relevant licenses or terms of use for external assets such as evaluated models, source corpora, and supporting software.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}{}
    \item[] Justification: In this work, we introduce a new dataset along with a new suite of domain specific metrics. The link to the code and dataset are provided in the submission.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not report crowdsourcing experiments or human-subject studies as part of the core benchmark contribution.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The current paper does not involve human-subject research requiring IRB review.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}
    \item[] Justification: The benchmark evaluates multiple AI co-scientist systems, and the validation section also includes pairwise LLM-judge experiments using Gemini-family models. The paper describes these uses as part of the methodology and empirical evaluation.
    
\end{enumerate}

